Differentiable Model Predictive Control on the GPU

Differentiable model predictive control (MPC) offers a powerful framework for combining learning and control. However, its adoption has been limited by the inherently sequential nature of traditional optimization algorithms, which are challenging to parallelize on modern computing hardware like GPUs. In this work, we tackle this bottleneck by introducing a GPU-accelerated differentiable optimization tool for MPC. This solver leverages sequential quadratic programming and a custom preconditioned conjugate gradient (PCG) routine with tridiagonal preconditioning to exploit the problem's structure and enable efficient parallelization. We demonstrate substantial speedups over CPU- and GPU-based baselines, significantly improving upon state-of-the-art training times on benchmark reinforcement learning and imitation learning tasks. Finally, we showcase the method on the challenging task of reinforcement learning for driving at the limits of handling, where it enables robust drifting of a Toyota Supra through water puddles.

==> figs/bench_table_B.tex <==
\pgfplotstableread{
Index Method          Forward   Backward
0 {theseus (GPU)}     0    0
1 {mpc.pytorch (GPU)} 2109.1    5161.8
2 {trajax (GPU)}      2573    5209.1
3 {diffmpc (GPU)}     4735.5     13233.8
4 {theseus (CPU)}     0         0
5 {mpc.pytorch (CPU)} 1895.9    4438.4
6 {trajax (CPU)}      1712.9       3291
7 {diffmpc (CPU)}     301.8    688.4
}\datatable



% Create columns with 8000 if zero, else original
\pgfplotstablecreatecol[
    create col/expr={
        (\thisrow{Forward}==0 ? 50000 : \thisrow{Forward})
    }
]{ForwardPlot}{\datatable}

\pgfplotstablecreatecol[
    create col/expr={
        (\thisrow{Backward}==0 ? 50000 : \thisrow{Backward})
    }
]{BackwardPlot}{\datatable}


\newcommand\cpulabel[1]{\begin{tabular}{c}{#1}\\(CPU)\end{tabular}}
\newcommand\gpulabel[1]{\begin{tabular}{c}{#1}\\(GPU)\end{tabular}}

\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=10pt,
    width=\textwidth,
    height=5cm,
    enlarge x limits=0.08,
    ymin=0,
    ymax=20000,
    ylabel={Time (ms)},
    xtick=data,
    xticklabels={
		\cpulabel{theseus},
		\cpulabel{mpc.pt},
		\cpulabel{trajax},
		\cpulabel{diffmpc},
		\gpulabel{theseus},
		\gpulabel{mpc.pt},
		\gpulabel{trajax},
		\gpulabel{diffmpc}   
    },
    xticklabel style={rotate=0, anchor=north},
    ymin=0,
    legend style={at={(1.0,1.0)},anchor=north east, draw=white},
    nodes near coords style={rotate=90, anchor=west},
    axis lines*=left,
]

% Forward bars: height from ForwardPlot, meta is Forward (original data)
\addplot+[
    fill=blue!30,
    nodes near coords={
        \pgfmathfloatparsenumber{\pgfplotspointmeta}
        \pgfmathfloatifflags{\pgfmathresult}{0}{
            $>$20000
        }{
            \pgfmathprintnumber[fixed,precision=0]{\pgfplotspointmeta}
        }
    },
] table[
    x=Index,
    y=ForwardPlot,
    meta=Forward
] {\datatable};

% Backward bars: height from BackwardPlot, meta is Backward
\addplot+[
    fill=red!30,
    nodes near coords={
        \pgfmathfloatparsenumber{\pgfplotspointmeta}%
        \pgfmathfloatifflags{\pgfmathresult}{0}{
            $>$20000
        }{
            \pgfmathprintnumber[fixed,precision=0]{\pgfplotspointmeta}
        }
    },
] table[
    x=Index,
    y=BackwardPlot,
    meta=Backward
] {\datatable};

\legend{Forward, Backward}
\end{axis}
\end{tikzpicture}

==> figs/bench_table_C.tex <==
\pgfplotstableread{
Index Method          Forward   Backward
0 {theseus (GPU)}     0    0
1 {mpc.pytorch (GPU)} 3568.9    7913.9
2 {trajax (GPU)}      1934.9    3932.9
3 {diffmpc (GPU)}     3334     5865.8
4 {theseus (CPU)}     8566.5    12178.8
5 {mpc.pytorch (CPU)} 3767.7    8745.99
6 {trajax (CPU)}      2029.3	       3913.4
7 {diffmpc (CPU)}     341.7    529.9
}\datatable		

% Create columns with 8000 if zero, else original
\pgfplotstablecreatecol[
    create col/expr={
        (\thisrow{Forward}==0 ? 50000 : \thisrow{Forward})
    }
]{ForwardPlot}{\datatable}

\pgfplotstablecreatecol[
    create col/expr={
        (\thisrow{Backward}==0 ? 50000 : \thisrow{Backward})
    }
]{BackwardPlot}{\datatable}


\newcommand\cpulabel[1]{\begin{tabular}{c}{#1}\\(CPU)\end{tabular}}
\newcommand\gpulabel[1]{\begin{tabular}{c}{#1}\\(GPU)\end{tabular}}

\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=10pt,
    width=\textwidth,
    height=5cm,
    enlarge x limits=0.08,
    ymin=0,
    ymax=20000,
    ylabel={Time (ms)},
    xtick=data,
    xticklabels={
		\cpulabel{theseus},
		\cpulabel{mpc.pt},
		\cpulabel{trajax},
		\cpulabel{diffmpc},
		\gpulabel{theseus},
		\gpulabel{mpc.pt},
		\gpulabel{trajax},
		\gpulabel{diffmpc}   
    },
    xticklabel style={rotate=0, anchor=north},
    ymin=0,
    legend style={at={(1.0,1.0)},anchor=north east, draw=white},
    nodes near coords style={rotate=90, anchor=west},
    axis lines*=left,
]

% Forward bars: height from ForwardPlot, meta is Forward (original data)
\addplot+[
    fill=blue!30,
    nodes near coords={
        \pgfmathfloatparsenumber{\pgfplotspointmeta}
        \pgfmathfloatifflags{\pgfmathresult}{0}{
            $>$20000
        }{
            \pgfmathprintnumber[fixed,precision=0]{\pgfplotspointmeta}
        }
    },
] table[
    x=Index,
    y=ForwardPlot,
    meta=Forward
] {\datatable};

% Backward bars: height from BackwardPlot, meta is Backward
\addplot+[
    fill=red!30,
    nodes near coords={
        \pgfmathfloatparsenumber{\pgfplotspointmeta}%
        \pgfmathfloatifflags{\pgfmathresult}{0}{
            $>$20000
        }{
            \pgfmathprintnumber[fixed,precision=0]{\pgfplotspointmeta}
        }
    },
] table[
    x=Index,
    y=BackwardPlot,
    meta=Backward
] {\datatable};

\legend{Forward, Backward}
\end{axis}
\end{tikzpicture}
